Higher categorical symmetries and gauging in two-dimensional spin systems

We present a framework to systematically investigate higher categorical symmetries in two-dimensional spin systems. Though exotic, such generalised symmetries have been shown to naturally arise as dual symmetries upon gauging invertible symmetries. Our framework relies on an approach to dualities whereby dual quantum lattice models only differ in a choice of module 2-category over some input fusion 2-category. Given an arbitrary two-dimensional spin system with an ordinary symmetry, we explain how to perform the (twisted) gauging of any of its sub-symmetries. We then demonstrate that the resulting model has a symmetry structure encoded into the Morita dual of the input fusion 2-category with respect to the corresponding module 2-category. We exemplify this approach by specialising to certain finite group generalisations of the transverse-field Ising model, for which we explicitly define lattice symmetry operators organised into fusion 2-categories of higher representations of higher groups.

==> _D8.tex <==
\subsection{$\msf D_8$ gauge model with $\TRep(\msf D_8)$ symmetry\label{sec:D8}}
The group $\msf D8$ is significantly richer than the previously studied examples as (i) it is non-Abelian and (ii) it has a large number of subgroups.
%
Gauging various subgroups delivers dual models with interesting symmetry structures that have non-invertible, higher-form and higher-group elements.
%
The symmetry TFT for all the symmetry structures that are related by discrete gaugings is the same, this implies an important lesson, i.e., the representation theory of these symmetry structures is isomorphic.
%
It is most convenient to approach the representation theory from the vantage point of $\TVect(\msf D_8)$ as we will detail in later sections.
%
As in earlier sections, we begin with a preliminary analysis of the group structure of $\msf D_8$, then move onto describing the group algebra $\mbb C[\msf D_8]$, which will serve as the local Hilbert space on which the models of interest will be defined. 

\newl {\bf {Group structure:}} There are multiple ways to present $\msf D_8$. 
%
We find it convenient to express it as a semi-direct product $\msf D_8= \mbb Z_2 \rtimes (\mbb Z_2 \times \mbb Z_2)$
\begin{equation}
    \msf D_8 = \big \langle x, a, b \ \big| \ x^2=a^2=b^2=1  \ \& \ xax=b  \big \rangle. 
    \label{eq:S3_presentation}
\end{equation}
We denote $ab=c$, which is also an order 2 element. 
%
Therefore $\msf D_8 =\left\{1,a,b,c,x,xa,xb,xc\right\}$.
%
The group $\msf D_8$ has four normal subgroups (other than the trivial group and the full group), which in this presentation take the following form. 
% 
There is $\mbb Z_2$ group generated by $c$.
%
There are two $\mathbb Z_{2}\times \mathbb Z_2$ subgroups generated by $\langle a,c\rangle $ and $\langle x,c\rangle $ respectively.
%
Finally, there is a $\mbb Z_4$ subgroup generated by $xa$.
%
Any group element can be expressed by the triple ${\bf{n}}:=(n_x,n_c,n_a)\in \mathbb Z_2^{3}$ (as a set), identified as 
\begin{equation}
    \msf g= x^{n_x}\cdot c^{n_c}\cdot a^{n_a}.
\end{equation}
Group composition rules are 
\begin{equation}
    \msf g \cdot \msf g'= (x^{n_x}\cdot c^{n_c}\cdot a^{n_a})\cdot (x^{n'_x}\cdot c^{n'_c}\cdot a^{n'_a})=(x^{n_x+n'_x}\cdot c^{n_c+n'_c+n_an'_x}\cdot a^{n_a+n'_a}).
\end{equation}
A $\msf D_{8}$ gauge connection on a (triangulated) manifold $\Sigma$ can correspondingly be described by the triple $(X,C,A) \in C^{1}(\Sigma,\mathbb Z_{2})^3$ which satisfy the cocycle conditions
\begin{equation}
    dX=0, \quad dC=A\cup X, \quad dA=0.
\end{equation}
In what follows, we will describe $\msf D_8$ gauge models whose Hilbert space can be spanned by elements $(X,C,A)$ satisfying these cocycle conditions. 

\newl {\bf {$\msf D_8$ Hilbert space:}} The Ising and gauge models whose symmetry structures we study are built on graphs with local Hilbert spaces assigned to the vertices and edges respectively.
%
The local Hilbert space in both cases is the group algebra 
\begin{equation}
    \mathbb C[\msf D_8] = \text{Span}_{\mbb C}\left\{|\msf g\rangle \quad | \quad \msf g= x^{n_x}\cdot c^{n_c}\cdot a^{n_a}\in \msf D_8 
    \right\}.
\end{equation}
%
We find it convenient to build the the space of linear operators $\mathcal L[\mathbb C[\msf D_8]]$ using tensor products of Pauli matrices.
%
To this end, we define
\begin{equation}
    \Gamma^{\mu\nu\rho}=\sigma^{\mu}\otimes \sigma^{\nu}\otimes \sigma^{\rho},
\end{equation}
where $\mu\in \left\{0,\dots,3\right\}$. 
%
The basis states $|x,c,a\rangle$ are the simultaneous eigenbasis of $\Gamma^{300}, \Gamma^{030}$ and $\Gamma^{003}$ such that
\begin{equation}
\begin{split}
    \Gamma^{300}|{\bf{n}}\rangle =&(-1)^{n_x} |{\bf{n}}\rangle, \\   \Gamma^{030}|{\bf{n}}\rangle =&(-1)^{n_c} |{\bf{n}}\rangle, \\
    \Gamma^{003}|{\bf{n}}\rangle =&(-1)^{n_a} |{\bf{n}}\rangle. 
\end{split}
\end{equation}
Next, we implement local operators $L^{\msf g}$ that implement the left action on the eigen-basis
\begin{equation}
    L^{\msf g}|\msf g'\ra=  | \msf g \cdot \msf g'\ra.
\end{equation}
The expressions for the operators $L^{\msf g}$ for $\msf g\in \left\{x,c,a\right\}$ are
\begin{equation}
    \begin{split}
        L^{a}=&\Gamma^{001}, \\
        L^{c}=&\Gamma^{010}, \\
        L^{x}=&\Gamma^{100}\left[
        \Gamma^{010}\left(\frac{1-\Gamma^{003}}{2}\right)
        + 
        \Gamma^{000}\left(\frac{1+\Gamma^{003}}{2}\right)
        \right].
    \end{split}
\end{equation}
Since these operators satisfy the $\msf D_8$ group relations, the rest of the $L^{\msf g}$ operators can be obtained. 
%
Note that these operators naturally realize the regular  representation on $\msf D_8$, whose representation matrices are $|\msf G|\times |\msf G|$ dimensional permutation matrices.
%
Consequently, the characters $\chi^{\text{reg}}(\msf g)=|\msf G|\delta_{\msf g,1}$.
%
It is straightforward to verify using the character orthogonality relations, that this representation is in fact decomposable into irreducible representations of $\msf D_{8}$. 
%
 Any irrep $\rho$ of dimension $\msf d_{\rho}$ appears exactly $\msf d_{\rho}$ times in the decomposition.
 \begin{equation}
     \chi^{\text{reg}}(\msf g)=\bigoplus_{\rho \in \text{irrep}}\msf d_{\rho} \chi^{\rho}(\msf g).
 \end{equation}
 We will use this fact later when studying the representation theory of the web of symmetry categories arising by gauging subgroups of $\msf D_8$.

 \newl {\bf {$\msf D_8$ Ising model and its symmetry category:}}

  \newl {\bf {$\msf D_8$ gauge model and its symmetry category:}}
